Short-term variability and mass loss in Be stars II. Physical taxonomy of photometric variability observed by the Kepler spacecraft

Context: [abbreviated] Aims: Kepler data of three known Be stars are re-visited to establish their pulsational nature and assess the properties of additional, non-pulsational variations. The three program stars turned out to be one inactive Be star, one active, continuously outbursting Be star, and one Be star transiting from a non-outbursting into an outbursting phase, thus forming an excellent sample to distill properties of Be stars in the various phases of their life-cycle. Methods: [abbreviated] Results: The short-term photometric variability of Be stars must be disentangled into a stellar and a circumstellar part. The stellar part is on the whole not different from what is seen in non-Be stars. However, some of the observed phenomena might be to be due to resonant mode coupling, a mechanism not typically considered for B-type stars. Short-term circumstellar variability comes in the form of either a group of relatively well-defined, short-lived frequencies during outbursts, which are called \v{S}tefl frequencies, and broad bumps in the power spectra, indicating aperiodic variability on a time scale similar to typical low-order $g$-mode pulsation frequencies, rather than true periodicity. Conclusions: From a stellar pulsation perspective, Be stars are rapidly rotating SPB stars, that is they pulsate in low order $g$-modes, even if the rapid rotation can project the observed frequencies into the traditional high-order $p$-mode regime above about 4 c/d. However, when a circumstellar disk is present, Be star power spectra are complicated by both cyclic, or periodic, and aperiodic circumstellar phenomena, possibly even dominating the power spectrum.

==> macros_tri.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Own macros
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Astronomical Variables and Observables 
%
\newcommand{\mstar}{\mbox{$M_{\star}$}\xspace}
\newcommand{\rstar}{\mbox{$R_{\star}$}\xspace}
\newcommand{\req}{\mbox{$R_{\mathrm{eq}}$}\xspace}
\newcommand{\rpole}{\mbox{$R_{\mathrm{pole}}$}\xspace}
\newcommand{\lstar}{\mbox{$L_{\star}$}\xspace}
%
\newcommand{\teff}{\mbox{$T_{\mathrm{eff}}$}\xspace}
\newcommand{\logg}{\mbox{$\log g $}\xspace}
\newcommand{\logeps}{\mbox{$\log\varepsilon$}\xspace} 
\newcommand{\mdot}{\mbox{$\dot{M}$}\xspace}
\newcommand{\vsys}{\mbox{$v_{\mathrm{sys}}$}\xspace}
\newcommand{\vrad}{\mbox{$v_{\mathrm{rad}}$}\xspace}
\newcommand{\vpuls}{\mbox{$v_{\mathrm{puls}}$}\xspace}
\newcommand{\vred}{\mbox{$v_{\mathrm{red}}$}\xspace}
\newcommand{\vviolet}{\mbox{$v_{\mathrm{violet}}$}\xspace}
\newcommand{\vinf}{\mbox{$v_\infty$}\xspace}
\newcommand{\vesc}{\mbox{$v_{\mathrm{esc}}$}\xspace}
\newcommand{\vsini}{\mbox{$v\sin i$}\xspace}
\newcommand{\vrot}{\mbox{$v_{\mathrm{rot}}$}\xspace}
\newcommand{\vcrit}{\mbox{$v_{\mathrm{crit}}$}\xspace}
\newcommand{\vkep}{\mbox{$v_{\mathrm{orb}}$}\xspace}

\newcommand{\omeang}{\mbox{$\omega$}\xspace}
\newcommand{\omelin}{\mbox{$\Upsilon$}\xspace} % as in Cranmer, 2006
\newcommand{\omeorb}{\mbox{$W$}\xspace}

%\newcommand{\wlam}{\mbox{$W_{\lambda}$}\xspace}
\newcommand{\wlam}{\mbox{$\mathit{EW}$}\xspace}
%\newcommand{\la}{\mbox{$\lambda$}\xspace}
\newcommand{\bz}{\mbox{$\langle{B_z}\rangle$}\xspace}

\newcommand{\vr}{\mbox{$V\!/R$}\xspace}
\newcommand{\bminv}{\mbox{$B\!-\!V$}\xspace}
\newcommand{\uminb}{\mbox{$U\!-\!B$}\xspace}
\newcommand{\vminr}{\mbox{$V\!-\!R$}\xspace}
%
%        Astronomical units
%
\newcommand{\Mstar}{\mstar}   % Not a unit, but a normalization quantity
\newcommand{\Rstar}{\rstar}   % Not a unit, but a normalization quantity
% Let's do as if the following were SI:
\newcommand{\Msun}{\mbox{${\mathrm M}_{\odot}$}\xspace}
\newcommand{\Rsun}{\mbox{${\mathrm R}_{\odot}$}\xspace}
\newcommand{\Lsun}{\mbox{${\mathrm L}_{\odot}$}\xspace}
\newcommand{\Myr}{\mbox{${\mathrm M}_{\odot}{\mathrm{yr}}^{-1}$}\xspace}
\newcommand{\micron}{\mbox{$\mu\mathrm{m}$}\xspace}
\newcommand{\gcm}{\mbox{$\mathrm{g\,cm}^{-3}$}\xspace}
\newcommand{\kms}{\mbox{${\mathrm{km\,s}}^{-1}$}\xspace}
%
\renewcommand{\deg}{\degree\xspace}
%
%       Spectral lines, ions and spectral
%
\newcommand{\LyB}{\mbox{{{Ly}}$\mathrm{\beta}$}\xspace}
\newcommand{\HA}{\mbox{{H}$\mathrm{\alpha}$}\xspace}
\newcommand{\HB}{\mbox{{H}$\mathrm{\beta}$}\xspace}
\newcommand{\HG}{\mbox{{H}$\mathrm{\gamma}$}\xspace}
\newcommand{\HD}{\mbox{{H}$\mathrm{\delta}$}\xspace}
\newcommand{\HE}{\mbox{{H}$\mathrm{\epsilon}$}\xspace}
\newcommand{\BrG}{\mbox{{Br}$\mathrm{\gamma}$}\xspace}
\newcommand{\Pa}[1]{\mbox{{Pa}$_{#1}$}\xspace}
%
\newcommand{\spec}[3]{\mbox{#1\,{\sc #2}\,$\lambda$#3}\xspace}
\newcommand{\specs}[3]{\mbox{#1\,{\sc #2}\,$\lambda\lambda$#3}\xspace}
%\newcommand{\ion}[2]{\mbox{#1\,{\sc #2}}\xspace}
%
\newcommand{\spt}[2]{\mbox{#1\,#2}\xspace}
%
%
%       Objects
%
\newcommand{\alpara}{\mbox{$\mathrm{\alpha}$}~Ara\xspace}
\newcommand{\alperi}{\mbox{$\mathrm{\alpha}$}~Eri\xspace}
\newcommand{\betcep}{\mbox{$\mathrm{\beta}$}~Cep\xspace}
\newcommand{\betlyr}{\mbox{$\mathrm{\beta}$}~Lyr\xspace}
\newcommand{\gamcas}{\mbox{$\mathrm{\gamma}$}~Cas\xspace}
\newcommand{\delsco}{\mbox{$\mathrm{\delta}$}~Sco\xspace}
\newcommand{\omeori}{\mbox{$\mathrm{\omega}$}~Ori\xspace}
\newcommand{\mucen}{\mbox{$\mathrm{\mu}$}~Cen\xspace}
\newcommand{\etacen}{\mbox{$\mathrm{\eta}$}~Cen\xspace}
\newcommand{\mulup}{\mbox{$\mathrm{\mu}$}~Lup\xspace}
\newcommand{\kaplup}{\mbox{$\mathrm{\kappa^1}$}~Lup\xspace}

\newcommand{\lameri}{\mbox{$\mathrm{\lambda}$}~Eri\xspace}
\newcommand{\omecma}{\mbox{$\mathrm{\omega}$}~CMa\xspace}
\newcommand{\kapcma}{\mbox{$\mathrm{\kappa}$}~CMa\xspace}
\newcommand{\epscap}{\mbox{$\mathrm{\epsilon}$}~Cap\xspace}
\newcommand{\zettau}{\mbox{$\mathrm{\zeta}$}~Tau\xspace}
\newcommand{\phiper}{\mbox{$\mathrm{\varphi}$}~Per\xspace}
\newcommand{\piaqr}{\mbox{$\mathrm{\pi}$}~Aqr\xspace}
\newcommand{\psiper}{\mbox{$\mathrm{\psi}$}~Per\xspace}
\newcommand{\feper}{\mbox{$48$}~Per\xspace}
\newcommand{\felib}{\mbox{$48$}~Lib\xspace}
\newcommand{\betcmi}{\mbox{$\mathrm{\beta}$}~CMi\xspace}
\newcommand{\delcen}{\mbox{$\mathrm{\delta}$}~Cen\xspace}
\newcommand{\etatau}{\mbox{$\mathrm{\eta}$}~Tau\xspace}
\newcommand{\kapdra}{\mbox{$\mathrm{\kappa}$}~Dra\xspace}
\newcommand{\pcar}{\mbox{$\mathrm{p}$}~Car\xspace}
\newcommand{\alpcol}{\mbox{$\mathrm{\alpha}$}~Col\xspace}
\newcommand{\xioph}{\mbox{$\mathrm{\chi}$}~Oph\xspace}
\newcommand{\upscyg}{\mbox{$\mathrm{\upsilon}$}~Cyg\xspace}
\newcommand{\betpsc}{\mbox{$\mathrm{\beta}$}~Psc\xspace}
\newcommand{\omicas}{\mbox{$\mathrm{\omicron}$}~Cas\xspace}
\newcommand{\sixcep}{\mbox{$\mathrm{6}$}~Cep\xspace}
\newcommand{\omiaqr}{\mbox{$\mathrm{\omicron}$}~Aqr\xspace}
\newcommand{\thecrb}{\mbox{$\mathrm{\vartheta}$}~CrB\xspace}
\newcommand{\onedel}{\mbox{$1$}~Del\xspace}
\newcommand{\betmon}{\mbox{$\beta^1$}~Mon\xspace}
\newcommand{\omecar}{\mbox{$\omega$}~Car\xspace}
%
\newcommand{\sth}{\mbox{StH$\alpha$}166\xspace}
\newcommand{\als}{\mbox{ALS}10705\xspace}
\newcommand{\hd}{\mbox{HD}186567\xspace}
%
% Codes, Models, Instruments
%
\newcommand{\bruce}{{\sc bruce/kylie}\xspace}
\newcommand{\hdust}{{\sc hdust}\xspace}
\newcommand{\fastrot}{{\sc fas\-trot}\xspace}
\newcommand{\charron}{{\sc charron}\xspace}
\newcommand{\bedisk}{{\sc bedisk}\xspace}
\newcommand{\simeca}{{\sc simeca}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Fancy stuff 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lgrey{\color{black!30!white}}
\def\grey{\color{black!60!white}}
\def\green{\color{green}}
\def\textgreen{\color{ForestGreen}}
\def\black{\color{black}}
\def\red{\color{red}}
\def\blue{\color{blue}}
\def\yellow{\color{yellow}}
\def\white{\color{white}}
\def\magenta{\color{magenta}}
\definecolor{beige}{HTML}{FFDF8C}
\def\beige{\color{beige}}
\def\gold{\color{Olive}}
%
\newcommand{\draft}[1]{{{\bf\sf\red Draft:}\grey\sf\ #1}\xspace}
\newcommand{\TRi}[1]{{{\bf\sf\red Rivi:}\grey\sf\ #1}\xspace}
%\newcommand{\TRi}[1]{{{}}}

